How Easy is It to Fool Your Multimodal LLMs? An Empirical Analysis on Deceptive Prompts

The remarkable advancements in Multimodal Large Language Models (MLLMs) have not rendered them immune to challenges, particularly in the context of handling deceptive information in prompts, thus producing hallucinated responses under such conditions. To quantitatively assess this vulnerability, we present MAD-Bench, a carefully curated benchmark that contains 1000 test samples divided into 5 categories, such as non-existent objects, count of objects, and spatial relationship. We provide a comprehensive analysis of popular MLLMs, ranging from GPT-4v, Reka, Gemini-Pro, to open-sourced models, such as LLaVA-NeXT and MiniCPM-Llama3. Empirically, we observe significant performance gaps between GPT-4o and other models; and previous robust instruction-tuned models are not effective on this new benchmark. While GPT-4o achieves 82.82% accuracy on MAD-Bench, the accuracy of any other model in our experiments ranges from 9% to 50%. We further propose a remedy that adds an additional paragraph to the deceptive prompts to encourage models to think twice before answering the question. Surprisingly, this simple method can even double the accuracy; however, the absolute numbers are still too low to be satisfactory. We hope MAD-Bench can serve as a valuable benchmark to stimulate further research to enhance model resilience against deceptive prompts.

==> tables/tab_main_results.tex <==
\begin{table*}[t!]
\centering\
\huge
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccc|c}
\hline
\multicolumn{2}{c|}{\textbf{Models}}                  & \textbf{\begin{tabular}[c]{@{}c@{}}Count of\\ Object\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Non-existent\\ Object\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Object\\ Attribute\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Scene\\ Understanding\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Text\\ Recognition\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Meta\\ Average\end{tabular}} \\ \hline

\multicolumn{1}{c|}{{M1}}                  & Ferret~\citep{you2023ferret}  &0.00\%&	3.00\%&	0.00	\%&9.57	\%&7.8 \%&3.85 \%  \\
\multicolumn{1}{c|}{}                  & Kosmos2~\citep{peng2023kosmos}  &13.12\% &	2.46\% &	12.50	\% &9.65\% &	9.80 \% & 3.92\%                                                                                                                    \\

\multicolumn{1}{c|}{}                  & Yi-VL-34b~\citep{ai2024yi} &12.90\%&	8.44\%&	20.83\%&	11.50\%&	0.00\% & 9.17 \%                                                                                                                    \\
\multicolumn{1}{c|}{}                    & mPLUG-Owl2~\citep{ye2023mplug}& 34.38\%	&15.45\%	&29.17\%	&23.64	&16.67\% & 17.41\% \\                                                      
\multicolumn{1}{c|}{}                    & MiniCPM-Llama3-v2.5~\citep{viscpm} & 31.25\%	&	17.96	\%	&12.50\%	&	20.00\%	&	22.00\%	& 18.69\%                                                       \\
\multicolumn{1}{c|}{}                    & Phi-3-vision~\citep{abdin2024phi3}     & 59.38\%	&	25.29\%	&	20.83\%	&	31.86\%	&	46.00 \%	&28.08\%  
\\
\multicolumn{1}{c|}{}                    &XComposer2-7b~\citep{internlmxcomposer2_4khd} & 56.25	\%	&29.88\%	&	29.17\%	&	30.43	\%	&27.45 \%	&30.65\% \\
\multicolumn{1}{c|}{}                    &InternVL-Chat-v1.5~\citep{chen2024far} & 56.25\%	&	36.22\%	&	26.09\%	&	32.46\%	&	49.0\%	& 36.86 \%	\\
\multicolumn{1}{c|}{}                    &LLaVA-NeXT-7b-vicuna~\citep{liu2024llavanext} & \textbf{68.75\%}	&39.43\%	&	20.83\%	&	51.30	\%	&28.00 \%	&40.73\% \\
\multicolumn{1}{c|}{}                    &DeepSeek-VL-7b-chat~\citep{lu2024deepseekvl} & 40.62\%	&	46.73\%	&	29.17\%	&	46.43	\%	&56.25 \%	&46.53\% \\
\multicolumn{1}{c|}{}                    &Idefics-2-8b~\citep{laurençon2024matters}  & \textbf{68.75\%}	&	51.81\%	&	20.83\%	&	40.00\%	&	21.57 \%	&48.69\% \\
\multicolumn{1}{c|}{}                    &LLaVA-NeXT-13b-vicuna~\citep{liu2024llavanext} & \textbf{68.75\%}	&	49.61\%	&	29.17\%	&	54.78\%	&	36.00 \%	&49.65\% \\
\multicolumn{1}{c|}{}                    &LLaVA-NeXT-34b~\citep{liu2024llavanext}  & 41.94	\%	&51.76	\%	&25.00	\%	&56.14	\%	&26.53 \%	&50.05\% \\
\multicolumn{1}{c|}{}                    &Qwen-VL-Chat~\citep{bai2023qwenvl}  & 45.16	\%	&77.52\%	&	43.48	\%	&74.34	\%	&55.10 \%	&74.24\% \\
\hline

\multicolumn{1}{c|}{{M3}} & Gemini-Pro \citep{geminiteam2023gemini}& 46.88\%	&	47.16\%	&	25.00	\%	&41.96\%	&	34.00\%	& 45.36\%                                                     \\
\multicolumn{1}{c|}{}                    &  Reka~\citep{rekateam2024reka} & 43.75\%	& 	46.08\%	& 	37.50	\%	& 51.30\%	& 	47.06\%	&  46.46\% \\
\multicolumn{1}{c|}{}                    & GPT-4o~\citep{gpt4o}     & 81.25\%	&	82.77\%	&	66.67	\%	&85.84\%	&	76.47\%		& 82.35\%\\
\multicolumn{1}{c|}{}                    & GPT-4V \citep{OpenAI2023GPT4TR}    & 51.61	\%	&\textbf{83.16\%}	&	\textbf{70.83\%}	&	\textbf{89.29\%}	&	\textbf{88.24\%}	& \textbf{82.82\%}
                                              \\ \hline
\end{tabular}%
}
\caption{Main results on MAD-Bench. M1 denotes open-sourced models. M2 denotes additional open-sourced models that aim to reduce hallucination. M3 denotes  state-of-the-art proprietary systems. ($\dagger$) The meta average of accuracy is weighted by the amount of data in each category.}
\label{tab:result-1}
%\vspace{-2mm}
\end{table*}

==> tables/tab_simple_method0.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccc|c}
\hline
\textbf{Models} & \textbf{\begin{tabular}[c]{@{}c@{}}Count of \\ Object\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Non-existent \\ Object\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Object \\ Attribute\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Scene \\ Understanding\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Text \\ Recognition\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Meta \\ Average\end{tabular}} \\ \hline


Phi-3-vision*    & 53.57\% (-5.81\%) & 50.54\% (+25.25\%)   & 37.50\% (16.67\%)  & 53.51\% (+21.65\%) & 66.00\% (+20\%)  & 51.46\% (23.38\%)     \\

DeepSeek-VL-7b-chat*    & 44.83\% (+4.21\%)   & 62.32\% (+15.59\%)     & 47.83\% (+18.66\%)    & 61.82\% (+15.39\%)  & 48.00\% (-8.25\%) & 60.64\% (+14.11\%)               \\

NeXT-13b-vicuna*  & \textbf{45.16\% (-23.59\%)  }       & 71.33\% (+21.72\%)            & 37.50\% (+8.33\%)         & 74.11\% (+19.33\%)            & 38.00\% (+2.00\%)             &   68.21\% (+18.56\%)    \\

MiniCPM-Llama3-v2.5*    & 16.67\% (-14.58\%)    & 85.85\% (+67.89\%)        & 62.50\% (+50.00\%)      & 86.61\% (+66.61\%) & 68.63\% (+46.63\%)     & 82.25\% (+63.56\%)        \\

GPT-4V*     & 41.38\% (-10.23\%)       & \textbf{93.86\% (+10.7\%)}            & \textbf{75.00\% (+4.17\%)}        &     \textbf{99.11\% (+9.82\%)}         &   \textbf{90.20\% (+1.96\%)}          &    \textbf{92.23\% (+9.41\%)}       \\ \hline
\end{tabular}%
}
\caption{Results on MAD-Bench after modifying the test prompt. 
}
\label{tab:result-0}
\vspace{-1mm}
\end{table*}

==> tex/8_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Benchmark data and evaluate code: \url{https://anonymous.4open.science/r/MAD-Bench-4A83/README.md}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
